Progressive Supervision via Label Decomposition: An Long-Term and Large-Scale Wireless Traffic Forecasting Method

Long-term and Large-scale Wireless Traffic Forecasting (LL-WTF) is pivotal for strategic network management and comprehensive planning on a macro scale. However, LL-WTF poses greater challenges than short-term ones due to the pronounced non-stationarity of extended wireless traffic and the vast number of nodes distributed at the city scale. To cope with this, we propose a Progressive Supervision method based on Label Decomposition (PSLD). Specifically, we first introduce a Random Subgraph Sampling (RSS) algorithm designed to sample a tractable subset from large-scale traffic data, thereby enabling efficient network training. Then, PSLD employs label decomposition to obtain multiple easy-to-learn components, which are learned progressively at shallow layers and combined at deep layers to effectively cope with the non-stationary problem raised by LL-WTF tasks. Finally, we compare the proposed method with various state-of-the-art (SOTA) methods on three large-scale WT datasets. Extensive experimental results demonstrate that the proposed PSLD significantly outperforms existing methods, with an average 2%, 4%, and 11% performance improvement on three WT datasets, respectively. In addition, we built an open source library for WT forecasting (WTFlib) to facilitate related research, which contains numerous SOTA methods and provides a strong benchmark.Experiments can be reproduced through https://github.com/Anoise/WTFlib.

==> texes/bios.tex <==
% \appendices
% \section{Proof of the First Zonklar Equation}
% Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
% \section{}
% Appendix two text goes here.


% use section* for acknowledgment
% \ifCLASSOPTIONcompsoc
%   % The Computer Society usually uses the plural form
%   \section*{Acknowledgments}
% \else
%   % regular IEEE prefers the singular form
%   \section*{Acknowledgment}
% \fi


% The authors would like to thank...


% Can use something like this to put references on a page
% by themselves when using endfloat and the captionsoff option.
% \ifCLASSOPTIONcaptionsoff
%   \newpage
% \fi

\vfill
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/MyPhoto.jpg}}]{Daojun Liang}
  received the B.S. degree in computer science from Taishan University, China, in 2016, and the M.S. degree from the School of Information Science \& Engineering from the Shandong Normal University, Jinan, China, in 2019. He is currently pursuing the Ph.D. degree with the School of Information Science and Engineering, Shandong University, Jinan, China.
  His research interests include deep learning, machine learning, time series forecasting and federated learning.
\end{IEEEbiography}
\vfill

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/HaixiaZhang.jpg}}]{Haixia Zhang}(Senior Member, IEEE) received the B.E. degree from the Department of Communication and Information Engineering, Guilin University of Electronic Technology, China, in 2001, and the M.Eng. and Ph.D. degrees in communication and information systems from the School of Information Science and Engineering, Shandong University, China, in 2004 and 2008, respectively. From 2006 to 2008, she was an Academic Assistant at the Institute for Circuit and Signal Processing, Munich University of Technology. From 2016 to 2017, she was a Visiting Professor with the University of Florida, USA. She is currently a Distinguished Professor with Shandong University. Her current research interests include industrial Internet of Things (IIoT), resource management, mobile edge computing, and smart communication technologies. She serves as a TPC member, a session chair, an invited speaker and a keynote speaker for conferences. She is on the Editorial Boards of the \textit{IEEE Transactions on Wireless Communications, IEEE Internet of Things Journal, IEEE Wireless Communication Letters}, and \textit{China Communications}.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/DongfengYuan.png}}]{Dongfeng Yuan}(Senior Member, IEEE) received the M.S. degree from the Department of Electrical Engineering, Shandong University, China, in 1988, and received the Ph.D. degree from the Department of Electrical Engineering, Tsinghua University, China, in January 2000. Currently, he is a full professor in the School of Civil Engineering, Shandong University, China. From 1993 to 1994, he was with the Electrical and Computer Department at the University of Calgary, Alberta, Canada. He was with the Department of Electrical Engineering in the University of Erlangen, Germany, from 1998 to 1999; with the Department of Electrical Engineering and Computer Science in the University of Michigan, Ann Arbor, USA, from 2001 to 2002; with the Department of Electrical Engineering in Munich University of Technology, Germany, in 2005; and with the Department of Electrical Engineering Heriot-Watt University, UK, in 2006. His current research interests include Intelligent communication systems, mobile edge computing and cloud computing, AI and big data processing for communications.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/xiaoyan_ma.jpg}}]{Xiaoyan Ma} received the B.S. degrees from the School of Information Science and Engineering, Shandong University, China, in 2017. She is currently pursuing her Ph.D. degree at the School of Information Science and Engineering, Shandong University, China. Her research interests include multiple-in multiple-out (MIMO) technology, reconfigurable intelligent surface (RIS) and machine learning.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/lidongyang.jpg}}]{Dongyang Li} received the B.E. and M.Eng. degrees in communication engineering from the School of Information Technology, Wuhan University of Technology, China, in 2015 and 2017, respectively. He is currently pursuing the Ph.D. degree with the School of Information Science and Engineering, Shandong University, China. His research interests include mobile edge computing, edge caching, federated learning, smart communication technologies.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/MinggaoZhang.png}}]{Minggao Zhang}
  received the B.Sc. degree in mathematics from Wuhan University, Wuhan, China, in 1962.  He was a Group Leader of the Radio Transmission Research Group, ITU-R, Geneva, Switzerland. He has been an Academician of Chinese Academy of Engineering, Beijing, China, since 1999. He is currently a Distinguished Professor with the School of Control Science and Engineering, Shandong University, Jinan, China, and a Senior Engineer of the 22nd Research Institute of China Electronics Technology Corporation, Xinxiang, China. He has been involved in the research of radio propagation for decades. Many of his proposals have been adopted by international standardization organizations, including CCIR P.617-1, ITU-R P.680-3, ITU-R P.531-5, ITUR P.529-2, and ITU-R P.676-3. Prof. Zhang is currently a fellow of the China Institute of Communications. He has received seven National and Ministerial Science and Technology awards in China. He has been an Academician with the Chinese Academy of Engineering since 1999. 
\end{IEEEbiography}


% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}
